Probing Particle Physics with IceCube

The IceCube observatory located at the South Pole is a cubic-kilometre optical Cherenkov telescope primarily designed for the detection of high-energy astrophysical neutrinos. IceCube became fully operational in 2010, after a seven-year construction phase, and reached a milestone in 2013 by the first observation of cosmic neutrinos in the TeV-PeV energy range. This observation does not only mark an important breakthrough in neutrino astronomy, but it also provides a new probe of particle physics related to neutrino production, mixing, and interaction. In this review we give an overview of the various possibilities how IceCube can address fundamental questions related to the phenomena of neutrino oscillations and interactions, the origin of dark matter, and the existence of exotic relic particles, like monopoles. We will summarize recent results and highlight future avenues.

==> sterile_neutrinos.tex <==
It is conceivable that the three neutrino flavour states, $\nu_e$, $\nu_\mu$, and $\nu_\tau$, are augmented by additional states. The number of light ``active'' neutrinos, {\it i.e.} neutrinos that take part in the Standard Model weak interactions is limited to the known flavour states from the observed decay width of the $Z$-boson. However, it is feasible that there are light ``sterile'' neutrinos states with no Standard Model interactions. These sterile states would imply the existence of additional neutrino mass eigenstates that could impact the three-flavour neutrino oscillation phenomenology, due to an extended PMNS mixing matrix $\widetilde{U}$,
\begin{equation}\label{eq:sterilenu}
  |\nu_\alpha\rangle =
  \sum_{j=1}^{3+n} \widetilde{U}_{\alpha j}^* |\nu_j\rangle\,.
\end{equation}
The term ``sterile'' referring to neutrinos was introduced by B. Pontecorvo already in 1968 when discussing the, at that time hypothetical, possibility of vacuum neutrino oscillations~\cite{Pontecorvo:1967fh}. 
   
Many extensions of the Standard Model that relate to the appearance of neutrino mass terms predict the existence of sterile neutrinos.   
%  Non-zero neutrino masses imply the possibility
For instance, the existence of right-handed neutrino fields, $\nu_{\rm R}$, could give neutrinos a mass through a Dirac term,
  $m_{\rm D}\bar\nu_D\nu_D$, after electroweak symmetry breaking with Dirac fields $\nu_D = \nu_L + \nu_R$. Such states would be ``neutral'' with respect to the standard model gauge interactions, and therefore sterile. However, the smallness of the neutrino masses would require unnaturally small Yukawa couplings. This can be remedied in {\it seesaw} models (see {\it e.g.}~Ref.~\cite{Mohapatra:2006gs}). Being electrically neutral, neutrinos can also be Majorana particles, {\it i.e.}~spinors that are identical to their charge-conjugate state, $\nu = \nu^c$. This allows to form two Majorana fields $\nu_{m} = \nu_L + \nu^c_R$ and $\nu_{M} = \nu_R + \nu^c_L$. In this case we can introduce two more Majorana mass terms, $m\bar{\nu}_{m}\nu_{m}/2$ and $M\bar{\nu}_{\rm M}\nu_{\rm M}/2$.
%  They would add a desired symmetry to 
%  the right-- and left--handed components of the fermion families, and provide quark-lepton chirality symmetry: for each quark 
%  there would be a lepton of similar chirality. 
%  Being electrically neutral, neutrinos can also have a Majorana mass $m_{\rm M}$ of, in principle, any value up to the GUT scale. 
In {\it seesaw} models the individual size of the mass terms are such that $m\ll m_D \ll M$.
After diagonalization of the neutrino mass matrix, the masses of active neutrinos are proportional to $m_i\simeq m_D^2/M$, which can explain the smallness of neutrino masses. However, in this case the sterile neutrinos will obtain a large mass scale that is unobservable in oscillation experiments.
  %If $m_{\rm M} \gg m_{\rm D}$, the mass eigenstates for the left and right neutrino components are proportional to $m_{\rm D}/m_{\rm M}$ 
 % and $m_{\rm M}$, respectively, and one can explain the smallness of the masses of the known active neutrinos.  
 On the other hand, for values of
  $m_{\rm D} \gg m\simeq M$ (``pseudo-Dirac'' case), the active and sterile state mass states are degenerate after diagonalization, leading to maximal mixing between the left (active) and right (sterile) states. 
  
 The minimal sterile neutrino model is a ``3+1''
  model where, in addition to the three standard weakly-interacting neutrino flavours, one additional heavier sterile neutrino state is added.
  Such a simple extension of the neutrino sector has been advocated to explain certain tensions between experimental results from
  accelerators~\cite{Athanassopoulos:1996jb,Aguilar:2001ty,Aguilar-Arevalo:2013pmq}, reactor~\cite{Mention:2011rk}, radio-chemical~\cite{Bahcall:1994bq} and the predictions from the standard three active flavour scenario. In the most general case, the introduction of one sterile neutrino adds six new parameters to the neutrino oscillation phenomenology~\cite{Kopp:2013vaa}: three mixing angles
  $\theta_{\rm 14}$, $\theta_{\rm 24}$,
  $\theta_{\rm 34}$, two CP--violating phases, $\delta_{\rm 14}$ and $\delta_{\rm 34}$, and one mass difference, $\Delta m^2_{\rm 41}$, where the
  indexes '1-3' stand for the known neutrino mass states and '4' for the sterile state. Although sterile neutrinos can not be detected directly,
  their existence can leave an imprint on the oscillation pattern of active neutrinos. The sterile neutrino modifies the oscillation pattern of
  the standard neutrinos since these can now undergo vacuum oscillations into the new state, with a probability that is proportional to the
  new mixing angles. The period of these oscillations can be small, smaller than the directional resolution of IceCube, and the net
  effect is then to distort the overall $\nu_{\mu}$ flux normalization with respect to the three-flavour case. An additional effect arises from the
  different interactions of flavours with matter when traversing the Earth. The new possibility to oscillate to a state that does not interact results in
  energy and angular dependent oscillation amplitudes that depend on the mixing angles but also on the new  $\Delta m^2_{\rm 41}$.
  More precisely, the comparison between the oscillation pattern in the ${\rm (energy, zenith)}$ phase space predicted by the sterile ``3+1'' model
  and the pattern seen in experimental data that IceCube exploits to set limits on the sterile mixing parameters. As for the standard oscillation case
  described in section~\ref{sec:std_oscillations}, searches for sterile neutrinos 
  in IceCube are based on the detection of the disappearance of muon neutrinos and are more sensitive to $\theta_{\rm 24}$. Therefore the choice of
  a simplified minimal mixing scenario where only $\theta_{\rm 24}$ is not zero is justified, and is indeed the approach followed in the analyses
  described below. Nonzero values of the weakly constrained $\theta_{\rm 34}$ within current limits would not significantly affect the results presented
  here~\cite{Lindner2016}. \par

   There have been several searches in the past at sub--TeV energies with neutrinos from the Sun, reactors, and accelerator setups (see e.g.~\cite{Kopp:2013vaa,Gonzalez-Garcia:2015qrr,Capozzi:2016vac} and references therein). 
  The large flux of atmospheric neutrinos that reach IceCube and the energy range of the detector allow to search for signatures of 
  anomalous $\nu_{\mu}+{\bar\nu_{\mu}}$ disappearance caused by oscillations to an sterile neutrino, $\nu_{\rm s}$, at TeV energies, 
 an energy not probed before. Furthermore, the DeepCore detector can extend the search  down to about 6~GeV, improving  
  previous limits from smaller detectors.\par

 
\begin{figure}[t]
%\begin{minipage}[t]{0.45\linewidth}
%\centering\includegraphics[width=\linewidth,height=0.85\linewidth]{plots/sterile/sterile_limits_prl117_2016.pdf}
\centering\includegraphics[width=\linewidth]{plots/sterile/FinalResult_plot_v3-eps-converted-to.pdf}
\caption[]{The 90\% and 99\% C.L. exclusion contour on the (sin$^2 2\theta_{24}$, $\Delta m^2_{41})$ plane (orange solid line).
The green and yellow bands contain 68\% and 95\%, respectively, of the 90\% contours in simulated
pseudo-experiments. The contours and bands are overlaid
on 90\% C.L. exclusions from the Super-Kamiokande, MINOS, MiniBooNE and CDHS experiments~\cite{Abe:2014gda,Adamson:2011ku,Cheng:2012yy,Dydak:1983zq}, and
the 99\% C.L. allowed region from global fits to appearance experiments including MiniBooNE and LSND, assuming
$|U_{e4}|^2$=0.0023~\cite{Kopp:2013vaa} and $|U_{e4}|^2$=0.0027~\cite{Conrad:2012qt}, respectively. Figure from~\cite{Aartsen:2016oqi}}
\label{fig:HE_sterile}
\end{figure}

\begin{figure}[t]
%\end{minipage}\hfill
%\begin{minipage}[t]{0.45\linewidth}
%\centering\includegraphics[width=\linewidth]{plots/sterile/LowE_sterile_nosideplots.pdf}
\centering\includegraphics[width=\linewidth]{plots/sterile/Result_exclusion_limits_proj_all_NMO.pdf}
\caption[]{The exclusion contours on the (sin$^2 \theta_{24}$, $|U_{\tau 4}|^2)$ plane at 90\% and 99\% C.L. (dark and light blue solid lines, respectively). 
The dash lines show results from the Super-Kamiokande~\cite{Abe:2014gda}. Figure from~\cite{Aartsen:2017bap}}
\label{fig:LE_sterile}
%\end{minipage}\hfill
\end{figure}

The analysis techniques are very similar to the search for standard oscillations and are based on
  comparing the equivalent oscillogram from figure~\ref{fig:oscillogram} for oscillations with an sterile component, to the measured
  data. 
  Although the low--energy tracks provide a quite short lever arm to reconstruct their direction  with precision, and the angular resolution of the
  analysis varies between 
  6$^\circ$ and 12$^\circ$, depending on energy. This is enough, though, to perform the analysis (see figure 5 in~\cite{Aartsen:2017bap}) since
  the differences in the oscillation pattern in the presence of a sterile neutrino can still be distinguished from the non-sterile
  case with such angular resolution. 
  At higher energies the analyses necessarily follow a slightly different approach since the tracks originate outside the
  detector and the energy deposited in the hadronic shower at the interaction vertex
  is not accessible. Such analyses use measured muon energies instead of neutrino energies, like the one presented in~\cite{Aartsen:2016oqi}.
  The muon energy is reconstructed from the light emission profile from stochastic energy losses of the muon along its trajectory~\cite{Aartsen:2013vja},
  achieving an energy resolution of $\sigma_{\rm log_{10}}(E_{\mu}/{\rm GeV})\sim 0.5$. Since at the energies of this analysis the muon track can be well
  reconstructed, the angular resolution reaches values between 0.2$^\circ$ and 0.8$^\circ$, depending on incoming angle. \par

  As with searches for standard oscillations, the aim is to reach a pure sample of atmospheric neutrinos to be able to compare the measured number
  of events as a function of angle and energy with the model prediction. None of the analyses detected a deviation from the expected standard oscillation
  scenario and,
  therefore, limits on the oscillation parameters which depend on the additional neutrino can be set. The low--energy analysis uses a 8$\times$8
  binned grid in the  ${\rm (energy, cos(zenith))}$ plane while, due to its higher energy resolution, the high--energy analysis uses a 10$\times$20
  binned grid. A log-likelihood approach is used to find the best fit to the data given the model parameters. Confidence levels are calculated from
  the difference between the profile log-likelihood and the log-likelihood at the best fit point.  
The results are illustrated in figures~\ref{fig:HE_sterile} and~\ref{fig:LE_sterile}. Figure~\ref{fig:HE_sterile} shows the result of the
high--energy analysis expressed in the $(\Delta m_{\rm 14}^2, \sin^2 2\theta_{\rm 24})$ plane. The figure shows the  90\%  confidence level
contour (orange line) compared with  90\% exclusions from previous disappearance searches [7-10]. The exclusion is compatible with the
sensitivity (green and yellow areas) calculated under the assumption of the no-sterile neutrino hypothesis. The result therefore disfavours
much of the parameter space of the ``3+1'' model. 
 On the other hand, figure~\ref{fig:LE_sterile} shows the results of an analysis using low-energy events (6~GeV to 60~GeV)
 contained in DeepCore.  The results are shown in the $(|U_{\tau 4}|^2,|U_{\mu 4}|^2)$ plane,
 where $|U_{\tau 4}|$ is defined as $\sin^2\theta_{34}\,\cos^2\theta_{34}$ and $|U_{\mu 4}|$ is just $\sin^2 \theta_{24}$. The best-fit value 
 of these elements of the mixing matrix are $|U_{\mu 4}|^2=0.0$ and $|U_{\tau 4}|^2=0.08$, while the 90\% confidence level limits on their
 values are still compatible with 0, $|U_{\mu 4}|^2 \leq 0.11$ and $|U_{\tau 4}|^2 \leq 0.15$.  Combinations of the parameters shown in the
  axes above the contours are disfavoured. The figure includes recent exclusion contour from Super-Kamiokande~\cite{Abe:2014gda}
 as a comparison.

